Rearchitecting Classification Frameworks For Increased Robustness

While generalizing well over natural inputs, neural networks are vulnerable to adversarial inputs. Existing defenses against adversarial inputs have largely been detached from the real world. These defenses also come at a cost to accuracy. Fortunately, there are invariances of an object that are its salient features; when we break them it will necessarily change the perception of the object. We find that applying invariants to the classification task makes robustness and accuracy feasible together. Two questions follow: how to extract and model these invariances? and how to design a classification paradigm that leverages these invariances to improve the robustness accuracy trade-off? The remainder of the paper discusses solutions to the aformenetioned questions.

==> Contents/brians_stuff.tex <==
\newpage
\section{PointNet}
\label{sec:pointnet}

% 150 examples each
We train a PointNet model\cite{} as our root classifier for our sign classification case study. We crop and label points from the KITTI dataset\cite{} for each sign with at least 32 points. The original distribution of labels for signs as seen in Table~\ref{table:pc_distribution} accounts for the lack of diamond-shaped signs using jittering and translation as modes of data augmentation. The resulting accuracy of our root classifier holds at 98.01\%, with the class accuracies displayed in Table~\ref{table:pc_accuracy}. We evaluate the robustness of our PointNet model by generating adversarial attacks, an approach done by Xiang et al.\cite{}. Using an adapted Carlini-Wagner $L_2$ attack, perturbations are generated to minimize the $L_2$ distance and the targeted class loss. We use 500 iterations on each attack batch and find the adversarial accuracy to be greater than 90\% in some classes while keeping an average $L_2$ distance of around 1. Table~\ref{table:pc_adv} contains the results. We find that our 32-point model is robust to the clustering attack as explored by Xiang et al. in all but one class. While the norm-bounded generated attacks are physically realizable, we argue that our approach results in the adversary's cost being increased through perceptibility and feasibility.

% \begin{table}[H]
% \small
% \begin{center}
%   \begin{tabular}{  p{1.5cm}  p{1.5cm}  p{1.5cm}  p{1.5cm} p{2cm}}
%     \toprule
%     \texbf{Output} & \textbf{Circle} & \textbf{Diamond} & \textbf{Triangle} &
%     \textbf{Inverted Triangle}\\
%     \midrule
%     Avg L2 & 1.032 & 0.636 & 0.386 & 1.059 \\
%     Adv Acc & 91.33\% & 32.00\% & 98.00\% & 89.33\% \\
%     \bottomrule
%     \end{tabular}
% \caption{Average L2 perturbation distance between original and adversarial points. The adversarial accuracy is the percentage of successfully generated targeted attacks.}
% \label{table:pc_adv}
% \end{center}
% \vspace*{-8mm}
% \end{table}


\begin{table}[H]
\small
\begin{center}
  \begin{tabular}{p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm}}
    \toprule
    \textbf{Eval Acc} & \textbf{Eval Avg Class Acc} & \textbf{Circle} & \textbf{Diamond} & \textbf{Triangle} & \textbf{Inverted Triangle} \\
    \midrule
    98.01 & 98.33 & 98.80 & 100.0 & 100.0 & 94.50
    \end{tabular}
\caption{The accuracy of our PointNet classifier trained on sign shapes.}
\label{table:pc_accuracy}
\end{center}
\end{table}

\begin{table}[H]
\small
\begin{center}
  \begin{tabular}{p{1.5cm} p{1cm} p{1cm} p{1cm} p{1cm}}
    \toprule
    \textbf{Data source} & \textbf{Circle} & \textbf{Diamond} & \textbf{Triangle} & \textbf{Inverted Triangle} \\
    \midrule
    Original & 645 & 12 & 82 & 374 \\
    Augmented & 1290 & 492 & 738 & 1122
    \end{tabular}
\caption{The distribution of labels among our point clouds before and after data augmentation.}
\label{table:pc_distribution}
\end{center}
\end{table}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{figures/scene_sign.png}
%     \caption{Left: A point cloud of a scene in a driving environment. Right: The cropped point cloud of the sign outlined in red in the scene.}
%     \label{fig:pc_scene}
% \end{figure}

==> Contents/evaluation.tex <==
\newpage
\section{Evaluation}
\label{sec:evaluation}

% can we rephrase the main objective to show that domain knowledge improves the Rob/Acc trade-off and that a straightforward and intuitive method of doing so is via hierarchical classification -brian
We demonstrate that hierarchical classification improves the robustness vs. accuracy trade-offs. In this section, we evaluate our hierarchical classification approach for two commonly used domain tasks: speaker identification and image classification. For both tasks, we utilize a feed forward architecture with the final softmax layer. Speaker identification typically utilizes a siamese architecture to compute the distance between an unknown sample and a predefined support set, though such an architecture is hard to retrofit to obtain a robustness certificate. Through our evaluation, we establish that the improvements in robustness are independent of the following:
\begin{enumerate}
    \item The exact methodology used to obtain the robust invariant features (we utilize an auxiliary modality, \lidar, to classify shapes in the road sign classification task)
    \item The model chosen for robust classification (we use a robust SVM for gender identification as the root classifier for speaker identification)
    \item The domain space of the classification task (we evaluate our approach for image classification, road sign classification, and speaker identification)
\end{enumerate}

\textcolor{red}{add major results to the bullet points for the 3 themes suggested}
Our experiments suggest that:

\begin{enumerate}
    \item The hierarchical classification approach improves the robustness vs. accuracy trade-off for the same model architecture. While maintaining a comparable natural accuracy, the proposed approach produces an increase in certified robustness\footnote{Used interchangeably with the robustness certificate of Cohen et al.~\cite{cohen2019certified}}.
    \item Extending the hierarchy using multiple invariants further improves robustness. In the case of road sign classification, we combine shape and location constraints to obtain an average increase of $>80\%$ for speed limit signs (which can be thought of as circular signs at a given geographic location).
    % \item The hierarchical classification approach improves the robustness vs. accuracy trade-off; for the same model architecture, while maintaining the same accuracy (if not better in some cases), the proposed approach produces an average increase in robustness\footnote{Used interchangeably with the robustness certificate of Cohen et al.~\cite{cohen2019certified}} by $>60\%$. %For some points under consideration, the increase in robustness is up to 2000 $\times$.
    % \item Extending the hierarchy using multiple invariants further improves robustness. In our case study, we combined shape and location constraints to obtain an average increase of $>80\%$ for speed limit signs (which can be thought of as circular signs at a given geographic location).
    % \item While it is conceivable to run various types of adversarial attacks on point clouds, the perturbation produced is not realizable in the real world. The generated perturbation (as discussed in Table \ref{table:adv_attacks}, Sec.~\ref{pcattacks}) translates to a maximum change of 260 cm in depth. While some of these attacks impractical, these are also far from imperceptible, and are not easy to physically realize.
    % \item There exist several approaches to generate physically realizable adversarial examples (specifically for road signs). However, these approaches, and several others (as discussed in Sec.~\ref{realizable}) fail in inhibiting robust feature extraction.
\end{enumerate}

% We stress that this case study does not represent ``the solution'' to completely protect against adversarial attacks in the physical world. Instead, it demonstrates that invariants significantly raise the bar for launching specific type of adversarial attacks. It does so while improving robustness at no harm to accuracy.   


\subsection{Road Sign Classification}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/road-signs.pdf}
  \caption{The hierarchy over the road signs from the GTSRB dataset.}
  \label{fig:road-sign-setup}
\end{figure}

To summarize our hierarchical approach, we classify road signs first based on their shapes at the root level (using a classifier trained using the ResNet-20 architecture~\cite{DBLP:journals/corr/HeZRS15}). By doing so, we are able to partition the label space into equivalence classes based on shapes (circular, triangular, octagonal, inverse triangular, or rectangular). Within each equivalence class \ie per-shape, we perform classification using a smoothed classifier (which also has the ResNet-20 architecture) to obtain the exact road sign. Note that we set the noise parameter $\sigma$ set to different values \ie $\sigma=0.25,0.5,1$ to better understand the trade-offs between robustness and accuracy. Figure~\ref{fig:road-sign-setup} contains a visual summary. Such a hierarchical classification encodes various priors about the classification task which are obtained from domain expertise about the classification problem at hand. By doing so, the classification pipeline is also interpretable. We train the root classifier using \lidar point clouds (\ie a different set of input features) of road signs to predict the shape. While conventional computer vision techniques can be used to extract the shape of an object from raw pixel values (in the absence of an additional input modality), these are not fool-proof \ie the inputs are easy to perturb~\cite{}. In this case study, we demonstrate that features robust to $p$-norm perturbations exist in the wild (as motivated by our threat model in \S~\ref{}); such features provide us robustness for {\em free}\footnote{This is under the assumption that the point cloud inputs are robust, and hard to perturb. We validate this empirically in Sec.~\ref{realizable}}. Additionally, the presence of \lidars in most autonomous vehicles further validates our choice. 

{\bf Datasets:} For our experiments, we use two datasets: the first is the German Traffic Sign Recognition Benchmark (GTSRB)~\cite{Stallkamp2012} which contains 51,840 cropped images of German road signs which belong to 43 classes; Fig.~\ref{fig:road-sign-setup} shows these classes. The second is the KITTI dataset which contains time-stamped location measurements, high-resolution images, and \lidar scans over a five-day recording period from an instrumented vehicle on the roads of Karlsruhe, Germany. We post-processed this dataset to (a) extract only cropped images of the road signs included in the GTSRB dataset, and (b) exract their corresponding \lidar depth maps. To do so, we retrained a YOLOv3 object detector~\cite{yolov3} to detect the German road signs using the German Traffic Sign Detection Benchmark (GTSDB) dataset~\cite{}. Thus, we obtained 3138 cropped images, their corresponding \lidar depth maps, and their labels. To verify our pipeline, we {\em manually verified the validity of all} these labels.

\subsubsection{Improving the robustness vs. accuracy trade-off}
\label{improvement}


\para{\bf A Robust Root Classifier:} As discussed earlier, our root classifier operates on point cloud data. Our threat model specifies the adversary's capabilities to make $p$-norm bounded perturbations to the road sign, or deface the road sign with specific stickers. Such attacks are the state-of-the-art in literature. Our experiments with road signs and a \textcolor{red}{LIDAR NAME} \lidar suggest that {\em large} perturbations (such as stickers) made on the road sign does not impact the road sign's point cloud. Thus, the point cloud features are robust to perturbations on the actual road sign. While the \lidar is susceptible to active attacks~\cite{Cao:2019:ASA:3319535.3339815}, such an attack is expensive to mount and beyond the capabilities of our passive adversary. Recent works show $p$-norm bounded adversarial attacks exist in the point cloud space\cite{point_perturb_generate}. To evaluate our approach, we attack our PointNet~\cite{pointnet} shape classifier, which has achieved a 98.01\% accuracy on the test set, using state of the art attacks. From the results shown in Table~\ref{table:pc_adv}, we show that generating perturbations minimizing the $L_2$ distance in the point cloud space is an effective attack. Our model is robust against the clustering attack, a result of traffic signs having very few points. While these norm-bounded attacks are physically realizable, they increase an adversary's cost of attack by introducing an additional attack space on top of the image space. In summary, we are able to utilize robust features obtained from another input modality to obtain a robust root classifier. 

% \begin{table}[H]
% \small
% \begin{center}
%   \begin{tabular}{p{2.1cm}  p{1cm}  p{1cm}  p{1cm} p{1cm}}
%     \toprule
%     \texbf{Output} & \textbf{Circle} & \textbf{Diamond} & \textbf{Triangle} &
%     \textbf{Inverted Triangle}\\
%     \midrule
%     Pert Avg L2 & 1.032 & 0.636 & 0.386 & 1.059 \\
%     Pert Adv Acc & 91.33\% & 32.00\% & 98.00\% & 89.33\% \\
%     Cluster Avg L2 & 1.000 & 0.000 & 0.000 & 0.000 \\
%     Cluster Adv Acc & 100.0\% & 00.00\% & 00.00\% & 00.00\% \\
%     \bottomrule
%     \end{tabular}
% \caption{Displays perturbation attack and clustering attack. Average L2 perturbation distance between original and adversarial points. The adversarial accuracy is the percentage of successfully generated targeted attacks.}
% \label{table:pc_adv}
% \end{center}
% \vspace*{-8mm}
% \end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/scene_sign.png}
    \caption{Left: A point cloud of a scene in a driving environment. Right: The cropped point cloud of the sign outlined in red in the scene.}
    \label{fig:pc_scene}
\end{figure}

\noindent{\em Q1. Why Shape?} \textcolor{red}{PENDING}

\para{\bf The Leaf Classifiers:} Based on the signs in the GTSRB dataset, we observe that the diamond, octagon, and inverse-triangle shapes have a single road sign belonging to each of their equivalence classes. Thus, for these shapes, we do not require a leaf classifier; classifying based on the robust feature is sufficient. Consequently, their robustness certificate is $\infty$. 

\noindent{\em Q2. Retraining vs. Renormalization?} Under the assumption of an accurate and robust root classifier, each leaf classifier only accepts as input road signs belonging to particular shape. As a running example, let us assume that the leaf classifier under discussion classifies {\em circular} road signs. To obtain such a leaf classifier, one could (a) utilize a classifier trained on all labels (henceforth referred to as the baseline classifier) and discard the probability estimates of the labels not of interest (\ie labels of road signs which are not circular), and renormalize the remaining probability estimates; we refer to such an approach as the {\em renormalization} approach, or (b) {\em retrain} a leaf classifier from scratch based on the labels belonging to that particular equivalence class; \eg retrain a classifier for circular road signs in particular. Appendix~\ref{} contains results from both these approaches. We observe that both these approaches increase the robustness certificate; while the renormalization approach can only increase the robustness certificate (by design), the retraining approach can potentially decrease the robustness certificate for some inputs.

Recall that the value of the robustness certificate is directly proportional to the margin $\Phi^{-1}(\underline{p_A})-\Phi^{-1}(\overline{p_B})$, which is dependent on the probability $p_A$ of the top class $c_A$, and probability $p_B$ of the runner-up class $c_B$. Two important observations guide our analysis: (1) Note that $c_B$ can either belong to the same equivalence class as $c_A$ (denoted $c_A \approx c_B$), or belong to a different equivalence class (denoted $c_A \napprox c_B$), and (2) The probability estimates for each of the leaf classifiers (which predict only a subset of the labels), before renormalization, are the same as those in the baseline classifier (by construction). On reducing the label space, if $c_A \approx c_B$, renormalization will further widen the margin, and increase the robustness certificate. If  $c_A \napprox c_B$, then there must exist a runner-up candidate $c_{B'} \approx c_A$. Its corresponding runner-up estimate $\overline{p_{B'}} \leq \overline{p_B}$ (or it would have been the runner-up in the first place). Consequently, the margin $\Phi^{-1}(\underline{p_A})-\Phi^{-1}(\overline{p_{B'}}) \geq \Phi^{-1}(\underline{p_A})-\Phi^{-1}(\overline{p_B})$. 

% Again, on renormalization, this margin widens further. \footnote{From our experiments, we observed that the probability estimates of labels that {\em do not belong to the equivalence class} are oftentimes zero. In such scenarios, renormalization of the probability estimates that belong to the equivalence class does not widen the margin, but keeps it the same as before. Consequently, the certificate also remains the same.}.

In the retraining scenario, however, we do not have knowledge about the {\em ordering} of the probability estimates in the retrained classifier in comparison to the baseline classifier. It is possible that for a retrained classifier and for a given input, while the correct class' estimate remains $\underline{p_A}$, the new runner-up's estimate $\overline{p_{B'}}$ can be greater, lesser, or equal to the original (baseline) estimate $\overline{p_B}$. Thus, the new robustness certificate can either be lower, greater, or the same as the baseline scenario. This problem is more fundamental; since robustness is a local property relying on the local Lipschitz constant and the structure of the decision spaces, partial or incomplete knowledge of any of these can result in spurious selection of the runner-up label. An added benefit of the renormalization approach is that it is computationally efficient; one needs to train one baseline classifier (independent of how the label space is partitioned) as opposed to several leaf classifiers (depending on the nature of the partition). \textcolor{red}{maybe more stuff to be added from german paper + tommi paper}


%\paragraph{Can we do better?} Since the reduction in the robustness certificate is dependent on the runner-up $B$, we attempted to constrain the selection of this class by introducing an additional class (\texttt{OTHER}) in the training process. The training data corresponding to the \texttt{OTHER} label was uniformly sub-sampled from all other equivalence classes. %We believed that if the \texttt{OTHER} class was chosen as the runner-up, this would replicate the scenario in the baseline class, and consequently cause less deterioration in the robustness certificate \textcolor{red}{improve the previous sentence}. However, our results (Figure \ref{}) suggests otherwise; 
%This problem is more fundamental - since robustness is a local property, relying on the local Lipschitz constant, and the structure of the decision spaces - partial or incomplete knowledge of any of these can result in spurious selection of $p_{B'}$. We leave determining a better strategy than our renormalization approach to future work.  


\begin{figure}[ht]
  \centering
  \includegraphics[width=0.55\linewidth]{figures/speedlimits_plot.pdf}
  \caption{The percentage improvement of the robustness certificate for \texttt{SpeedLimit} signs utilizing a 2 layer hierarchical classifier. These results are a significant improvement on those of Fig.~\ref{fig:renormorretrain}}
  \label{fig:speedlimits}
\end{figure}


\subsubsection{Adding More Invariants}
\label{sec:morerobustfeatures}
%@kassem: certified accuracy for these points
%.25: 75
%.5 : 56.41
%1: 39.75

%Consider the following scenario: using the geographical coordinates, an autonomous vehicle is able to query a database to obtain the nature of the road it is on (\eg if the road is a highway, or an intersection etc.). 
Using location information, one is able to again partition the label space. For example, a highway can not have stop signs, or an intersection will not have a speed limit sign etc. To validate this hypothesis, we performed a small scale proof-of-concept experiment to further constrain the space of labels that is obtained by splitting on the shape feature (\ie see if we can obtain a subset of the set of, say, circular labels). Using the location information from the KITTI dataset, and local map data from OpenStreetMap \cite{OSM}, %we observe that: (a) different speed limit signs are often co-located geographically, (b) speed limit signs of 70kmph and below are geographically co-located, and (c) speed limit signs of 80kmph and above are geographically co-located with one way roads. Based on insight (a), 
for particular locations, we can further constrain the space of circular road signs to just \texttt{SpeedLimit} signs. From Fig.~\ref{fig:speedlimits}, we observe that increasing the number of robust features (to 2 - shape {\em and location}) increases the robustness certificate further. The ordering of robust features in the hierarchy (\eg shape followed by location vs. location followed by shape) to obtain the best increase in robustness is an open question, one which we wish to tackle in future work. 

\subsection{Speaker Identification}

Conventional speaker identification systems utilize a siamese architecture; speech samples are first converted to discrete features~\cite{}, and these are then converted to an embedding. The distance between an unknown embedding (which is to be labeled), and embeddings in a known support set are computed. The label of the known embedding in the support set which is at the least distance from the unknown embedding is returned as the label for the unknown sample. Observe that such an architecture is not conducive for computing certificates using randomized smoothing; the output returned by the network is a label, and there is no associated probability estimate for this prediction. Thus, we implement speaker identification using a conventional feed-forward architecture \textcolor{red}{describe specifics}. For the remainder of this section, we assume that the inputs are discrete features obtained after processing the voice samples.

As before, we classify inputs based on the gender of the speaker\textcolor{red}{nicolas wants to talk about the privacy implications of doing so.}. Since gender is binary, we utilize a robust SVM~\cite{} for this task. Unlike the previous case study where the root is robust to perturbation as its inputs are robust, the robustness guarantees for this case study come from the design of the classifier. We chose to use a SVM because of the nature of the classification (binary) as well as insights from prior work which suggest that the male and female speakers are linearly separable in some higher dimension~\cite{}. While we could utilize another modality to obtain speaker gender, we use a robust classifier to highlight the flexibility of our approach. As before, the leafs are trained using a smoothed classifier whose architecture is specified earlier. 

{\bf Datasets:} For our experiments, we use the LibriSpeech ASR corpus~\cite{}
